Decentralized State Estimation In A Dimension-Reduced Linear Regression

Decentralized state estimation in a communication-constrained sensor network is considered. The exchanged estimates are dimension-reduced to reduce the communication load using a linear mapping to a lower-dimensional space. The mean squared error optimal linear mapping depends on the particular estimation method used. Several dimension-reducing algorithms are proposed, where each algorithm corresponds to a commonly applied decentralized estimation method. All except one of the algorithms are shown to be optimal. For the remaining algorithm, we provide a convergence analysis where it is theoretically shown that this algorithm converges to a stationary point and numerically shown that the convergence rate is fast. A message-encoding solution is proposed that allows for efficient communication when using the proposed dimension reduction techniques. We also derive different properties from the proposed framework and show its superiority in relation to baseline methods. The applicability of the different algorithms is demonstrated using a simple fusion example and a more realistic target tracking scenario.

==> fig/data/data__evaluation_dtt_trajectory.tex <==
\drawtraj{(0.095,-0.078)(3.086,-11.322)(8.264,-23.598)(12.478,-34.164)(14.976,-44.356)(16.414,-52.578)(16.651,-63.687)(17.506,-74.133)(17.695,-84.162)(15.842,-94.226)(11.500,-104.033)(6.718,-117.731)(1.314,-131.891)(-5.615,-145.114)(-11.000,-155.986)};
\drawtraj{(0.079,0.104)(6.644,-4.486)(14.963,-9.756)(24.332,-16.034)(33.514,-20.639)(43.749,-26.681)(53.385,-32.477)(61.107,-37.116)(67.864,-41.932)(74.317,-46.941)(79.471,-51.687)(83.566,-56.277)(85.455,-61.667)(84.672,-68.968)(83.602,-77.678)};
\drawtraj{(-0.086,0.137)(6.473,3.986)(14.901,8.246)(23.649,13.670)(32.093,18.722)(43.031,23.596)(55.293,28.332)(65.973,33.521)(76.355,39.907)(85.637,45.591)(93.232,53.156)(102.159,63.187)(110.798,73.215)(116.935,83.396)(123.268,93.948)};
\drawtraj{(0.005,-0.156)(-18.529,8.440)(-38.891,18.206)(-60.062,31.783)(-83.309,45.598)(-102.573,56.377)(-120.957,66.698)(-137.859,76.738)(-157.658,86.237)(-180.275,93.847)(-201.888,100.873)(-222.491,109.018)(-243.388,117.782)(-263.144,129.369)(-283.666,141.727)};
\drawtraj{(0.135,0.118)(8.620,-14.924)(14.561,-28.761)(16.758,-41.135)(18.830,-53.816)(24.692,-65.653)(32.434,-75.675)(39.973,-83.689)(46.153,-90.720)(53.300,-95.650)(62.782,-98.324)(72.697,-99.672)(86.106,-99.611)(100.002,-100.064)(113.799,-102.788)};
\drawtraj{(0.046,-0.129)(-13.404,8.433)(-25.823,16.293)(-37.743,20.506)(-47.110,22.500)(-54.678,21.164)(-62.989,20.177)(-72.823,18.010)(-82.032,20.320)(-90.272,23.188)(-97.815,24.917)(-103.237,26.945)(-108.944,27.820)(-116.167,28.179)(-123.110,25.960)};
\drawtraj{(0.068,0.028)(0.668,11.126)(0.306,24.016)(1.697,35.660)(2.622,45.682)(5.684,57.081)(7.420,71.661)(9.707,84.533)(14.744,98.193)(17.735,113.656)(18.282,132.822)(17.424,150.900)(15.956,169.799)(14.025,188.599)(12.604,206.626)};
\drawtraj{(0.050,-0.058)(-2.443,-11.045)(-7.030,-22.096)(-11.493,-35.833)(-9.988,-49.922)(-7.594,-63.544)(-6.324,-77.708)(-6.385,-94.814)(-5.532,-114.021)(-2.831,-133.018)(0.469,-154.194)(3.417,-174.008)(6.016,-194.809)(8.987,-213.146)(12.150,-229.391)};
\drawtraj{(-0.076,-0.026)(-1.261,5.633)(-4.730,10.495)(-7.450,15.203)(-8.787,21.424)(-13.514,29.527)(-20.749,37.754)(-28.326,44.328)(-35.409,51.416)(-41.412,57.327)(-46.346,64.247)(-50.619,72.653)(-54.561,84.275)(-55.645,96.507)(-56.778,112.814)};
\drawtraj{(0.151,-0.110)(0.232,19.232)(1.512,37.732)(3.202,53.899)(4.430,69.865)(6.176,83.499)(7.536,95.322)(6.099,106.958)(4.414,117.405)(-0.710,130.258)(-5.902,142.273)(-11.693,153.814)(-14.623,167.990)(-13.757,183.598)(-11.377,202.258)};
\drawtraj{(-0.063,0.052)(-1.473,7.637)(-2.314,13.845)(-2.663,21.398)(-1.308,30.981)(0.953,40.167)(2.174,48.586)(2.364,57.361)(2.669,66.148)(4.226,75.264)(7.529,83.651)(8.446,92.206)(8.351,99.799)(7.407,111.757)(6.189,126.910)};
\drawtraj{(-0.057,0.083)(11.930,19.905)(22.428,39.461)(32.186,60.639)(40.363,83.304)(47.473,106.941)(56.316,129.084)(67.990,153.173)(78.763,176.992)(88.346,202.511)(98.464,227.799)(109.729,253.733)(120.469,279.176)(129.510,302.699)(138.920,324.362)};
\drawtraj{(-0.172,-0.186)(4.016,-11.877)(6.611,-21.227)(11.043,-30.860)(15.741,-39.973)(18.760,-50.259)(20.969,-62.892)(24.760,-78.311)(27.599,-92.759)(29.551,-107.688)(31.768,-124.554)(35.975,-140.695)(41.838,-159.128)(49.392,-177.936)(58.937,-194.482)};
\drawtraj{(0.062,0.123)(-3.543,-5.589)(-5.460,-11.598)(-7.552,-16.785)(-7.706,-20.961)(-8.173,-25.045)(-10.250,-28.014)(-10.557,-29.468)(-10.822,-31.489)(-11.956,-32.141)(-13.993,-31.738)(-15.408,-32.101)(-14.597,-34.953)(-13.431,-38.419)(-9.048,-41.814)};
\drawtraj{(-0.156,-0.193)(2.565,-7.118)(5.351,-17.174)(6.016,-27.207)(7.528,-36.667)(8.674,-48.238)(8.391,-61.908)(9.953,-74.831)(13.221,-85.616)(14.732,-96.465)(13.274,-107.762)(9.872,-120.302)(5.819,-131.557)(3.693,-144.165)(1.959,-154.688)};
\drawtraj{(0.093,0.024)(-14.592,-11.314)(-29.218,-23.396)(-41.281,-35.596)(-53.622,-50.204)(-66.997,-63.946)(-77.978,-78.859)(-90.099,-95.651)(-105.792,-113.121)(-119.859,-130.035)(-132.825,-146.726)(-148.977,-162.468)(-164.820,-176.680)(-180.592,-189.590)(-192.876,-201.147)};
\drawtraj{(0.036,0.136)(3.153,-1.046)(7.046,-2.355)(10.707,-1.754)(11.434,0.249)(8.292,3.855)(5.587,6.701)(2.507,7.241)(-0.040,7.345)(-1.334,7.464)(-4.427,7.192)(-5.384,6.901)(-8.085,10.624)(-13.494,14.149)(-19.664,15.603)};
\drawtraj{(0.100,-0.035)(-3.390,-4.551)(-6.612,-10.370)(-9.595,-17.525)(-11.185,-24.879)(-10.807,-31.997)(-9.742,-42.917)(-8.778,-52.154)(-7.708,-57.948)(-8.054,-65.073)(-7.267,-73.525)(-6.218,-82.412)(-3.760,-90.444)(1.501,-101.070)(6.793,-115.276)};
\drawtraj{(0.126,-0.032)(29.375,-20.786)(58.799,-38.548)(89.596,-54.824)(123.209,-68.697)(158.532,-78.414)(193.562,-85.120)(230.840,-90.834)(269.161,-93.951)(307.137,-97.821)(342.224,-104.523)(376.241,-112.130)(412.160,-119.025)(449.546,-125.693)(489.502,-131.378)};
\drawtraj{(-0.038,0.058)(7.610,9.287)(15.682,19.356)(26.074,32.002)(34.360,48.117)(43.853,65.909)(54.391,83.566)(64.590,103.093)(74.562,122.870)(82.058,141.315)(88.910,159.454)(94.629,176.284)(101.681,192.857)(109.329,209.136)(116.472,225.857)};
\drawtraj{(-0.112,-0.057)(-11.955,3.607)(-26.459,5.104)(-41.523,6.125)(-58.107,8.615)(-75.358,10.757)(-95.465,11.518)(-115.950,11.700)(-138.867,12.680)(-162.764,16.950)(-188.508,20.993)(-217.293,24.558)(-249.856,30.774)(-283.493,38.896)(-316.251,47.926)};
\drawtraj{(0.007,-0.040)(16.541,0.483)(34.120,-1.947)(50.449,-4.368)(63.836,-7.581)(78.050,-10.947)(92.876,-16.979)(108.486,-20.853)(124.126,-25.617)(139.483,-29.373)(154.731,-29.971)(170.660,-31.124)(183.986,-30.524)(195.762,-28.164)(204.089,-24.120)};
\drawtraj{(-0.024,0.094)(-3.682,-9.396)(-7.362,-18.369)(-12.004,-27.003)(-16.894,-34.498)(-20.107,-42.874)(-24.519,-51.041)(-31.010,-56.537)(-39.237,-59.974)(-45.499,-64.895)(-50.618,-70.657)(-57.644,-78.947)(-65.997,-87.557)(-73.973,-96.598)(-82.434,-108.078)};
\drawtraj{(0.157,0.032)(-4.566,17.137)(-6.725,34.214)(-5.376,54.945)(-4.296,76.770)(-2.677,97.560)(-1.389,116.016)(-2.727,134.248)(-4.243,151.521)(-6.861,168.227)(-10.032,183.862)(-11.776,198.807)(-13.165,214.160)(-13.208,230.627)(-11.693,249.169)};
\drawtraj{(0.027,-0.107)(15.795,17.388)(31.174,36.570)(46.118,55.436)(61.792,73.600)(75.941,91.024)(89.497,110.524)(103.311,129.222)(115.630,145.724)(128.393,162.464)(140.786,180.968)(156.243,201.860)(171.504,224.849)(189.130,247.077)(205.886,268.282)};
\drawtraj{(0.105,-0.049)(3.355,0.134)(5.595,0.352)(7.155,2.183)(8.693,6.370)(8.324,12.292)(8.991,19.698)(10.149,29.523)(9.707,40.732)(9.536,50.206)(11.673,58.824)(13.013,68.224)(12.849,76.415)(15.720,84.565)(22.151,93.710)};
\drawtraj{(-0.105,0.080)(-16.155,-13.739)(-30.573,-28.552)(-45.090,-44.004)(-60.829,-58.403)(-76.629,-74.644)(-91.400,-93.965)(-108.710,-112.801)(-129.911,-131.008)(-154.289,-148.866)(-179.566,-164.737)(-202.389,-182.224)(-224.766,-201.400)(-246.688,-220.975)(-268.240,-241.777)};
\drawtraj{(0.091,0.017)(2.441,11.497)(3.306,23.699)(2.487,36.319)(0.517,48.456)(-5.804,61.286)(-15.232,73.886)(-28.000,86.856)(-41.121,98.024)(-55.344,109.682)(-71.061,122.549)(-86.541,136.811)(-101.806,152.748)(-117.270,168.161)(-130.180,183.937)};
\drawtraj{(-0.041,0.023)(-24.989,8.859)(-49.990,16.865)(-75.277,22.620)(-100.597,31.364)(-124.682,39.185)(-146.926,49.471)(-168.292,59.263)(-190.375,66.858)(-212.402,75.114)(-235.345,85.368)(-257.907,92.231)(-280.023,100.194)(-303.078,110.258)(-326.854,120.177)};
\drawtraj{(-0.051,-0.132)(11.872,1.308)(22.340,3.340)(29.497,7.365)(35.568,12.547)(39.699,18.576)(42.734,24.523)(44.380,30.367)(46.903,33.797)(47.514,33.455)(46.879,32.186)(43.877,28.982)(41.712,25.671)(38.507,20.567)(34.419,15.593)};
\drawtraj{(0.041,-0.014)(-8.319,-5.598)(-16.200,-11.349)(-25.474,-15.066)(-33.479,-18.900)(-37.033,-22.546)(-39.208,-28.450)(-41.646,-36.488)(-47.724,-47.154)(-52.897,-59.699)(-54.813,-70.134)(-55.263,-80.364)(-54.685,-88.931)(-53.498,-98.611)(-50.903,-110.447)};
\drawtraj{(-0.024,0.067)(-20.938,-3.076)(-43.846,-8.322)(-69.121,-13.534)(-97.336,-18.554)(-126.371,-22.009)(-156.104,-25.557)(-188.580,-30.250)(-220.822,-35.683)(-248.437,-40.920)(-276.365,-42.980)(-304.171,-44.441)(-329.900,-47.268)(-354.792,-46.307)(-380.473,-43.631)};
\drawtraj{(0.011,-0.130)(-0.785,19.145)(-4.131,39.227)(-8.388,57.176)(-12.238,71.991)(-17.763,83.573)(-25.472,93.191)(-32.940,104.043)(-40.770,116.003)(-50.390,127.673)(-60.430,141.201)(-68.332,155.509)(-75.146,170.506)(-81.502,184.899)(-84.699,198.736)};
\drawtraj{(-0.012,-0.070)(-1.471,-3.730)(-3.581,-8.823)(-2.793,-13.425)(-1.473,-18.194)(0.101,-24.898)(2.153,-27.035)(4.445,-30.642)(5.818,-34.532)(7.985,-36.599)(9.722,-38.277)(11.047,-41.000)(14.343,-42.446)(20.257,-44.532)(25.558,-46.069)};
\drawtraj{(-0.047,0.030)(10.444,4.709)(21.464,11.480)(34.103,17.450)(45.730,21.056)(55.617,26.533)(67.277,31.143)(79.204,36.525)(90.772,40.820)(100.918,44.412)(111.345,45.974)(122.614,49.106)(132.796,52.781)(142.922,54.435)(151.285,55.269)};
\drawtraj{(-0.070,0.066)(-2.233,-2.092)(-3.710,-6.314)(-4.661,-13.124)(-7.363,-19.278)(-11.102,-22.266)(-14.281,-26.137)(-17.806,-30.841)(-22.375,-35.112)(-28.324,-41.439)(-33.795,-47.788)(-40.675,-53.062)(-50.434,-60.119)(-59.799,-68.650)(-68.761,-75.911)};
\drawtraj{(-0.076,-0.014)(-7.453,3.751)(-17.439,4.244)(-27.838,1.814)(-38.073,0.431)(-48.390,1.463)(-55.167,1.872)(-62.113,5.543)(-69.106,11.253)(-74.807,18.419)(-77.464,26.272)(-80.329,36.008)(-85.681,45.636)(-90.904,54.815)(-97.672,65.406)};
\drawtraj{(-0.128,-0.097)(10.352,-14.516)(24.911,-30.561)(41.165,-42.778)(58.926,-51.526)(79.567,-61.433)(100.174,-72.330)(122.086,-80.387)(141.733,-90.706)(156.990,-101.387)(171.842,-114.061)(185.301,-128.455)(197.115,-144.086)(208.062,-157.526)(220.105,-168.992)};
\drawtraj{(-0.148,0.035)(-2.313,-12.227)(-5.164,-22.211)(-10.265,-31.575)(-16.496,-40.953)(-21.707,-49.080)(-24.669,-55.163)(-28.350,-61.010)(-32.284,-68.087)(-36.539,-75.289)(-40.149,-83.141)(-43.663,-90.170)(-50.053,-97.056)(-56.466,-105.928)(-61.735,-114.297)};
\drawtraj{(0.094,-0.021)(-0.318,7.012)(-1.244,18.744)(-3.906,30.046)(-8.268,41.403)(-12.759,53.368)(-18.714,66.526)(-24.454,80.552)(-31.339,94.291)(-37.858,104.667)(-42.973,115.602)(-50.802,128.329)(-58.595,140.095)(-68.533,152.781)(-78.754,167.147)};
\drawtraj{(-0.053,0.062)(16.666,-4.002)(31.952,-7.554)(46.862,-12.141)(60.481,-16.940)(75.504,-23.369)(91.322,-27.296)(106.993,-28.093)(120.973,-26.627)(135.857,-25.102)(149.336,-24.510)(162.073,-23.603)(179.491,-20.998)(197.932,-17.669)(216.630,-12.306)};
\drawtraj{(0.154,0.049)(-2.194,2.540)(-7.385,4.588)(-14.331,6.430)(-21.654,11.229)(-29.889,15.910)(-40.942,21.992)(-51.963,30.796)(-66.392,40.916)(-83.394,51.173)(-99.954,59.524)(-117.121,65.873)(-135.460,71.931)(-153.353,78.581)(-172.995,86.830)};
\drawtraj{(-0.107,-0.151)(9.017,10.190)(17.275,21.036)(25.956,30.791)(35.322,40.998)(47.270,50.721)(58.666,59.926)(71.088,68.689)(83.774,79.594)(95.055,90.090)(103.100,100.468)(107.930,109.462)(114.461,119.471)(122.789,131.111)(134.453,141.851)};
\drawtraj{(-0.126,-0.035)(-8.368,15.454)(-15.753,32.879)(-24.387,53.148)(-31.826,74.220)(-39.010,95.023)(-49.032,116.195)(-59.640,137.659)(-68.847,161.274)(-78.393,184.332)(-89.408,208.643)(-99.931,232.608)(-109.073,258.956)(-115.382,285.846)(-119.675,313.477)};
\drawtraj{(0.058,0.042)(0.972,-7.231)(2.892,-14.763)(3.796,-20.963)(4.729,-26.650)(7.265,-32.038)(10.007,-36.356)(10.122,-38.149)(11.388,-38.940)(12.824,-37.985)(15.313,-33.169)(17.776,-28.250)(21.178,-23.463)(24.673,-19.695)(26.656,-18.300)};
\drawtraj{(-0.013,-0.016)(-2.119,-2.110)(-3.690,-1.534)(-5.473,-0.132)(-6.802,-1.450)(-11.404,-7.285)(-19.581,-14.208)(-28.151,-19.335)(-35.900,-25.056)(-43.066,-31.786)(-47.122,-36.617)(-53.824,-41.868)(-60.778,-48.002)(-67.248,-54.229)(-73.836,-62.083)};
\drawtraj{(-0.070,0.082)(2.132,-2.363)(3.061,-4.607)(3.759,-10.800)(3.759,-17.490)(4.644,-22.947)(3.572,-26.990)(2.946,-32.535)(1.859,-38.023)(4.071,-45.253)(7.867,-52.264)(12.581,-58.316)(17.526,-65.589)(20.906,-73.385)(22.029,-80.559)};
\drawtraj{(0.026,-0.118)(-10.546,-5.442)(-20.107,-10.621)(-30.250,-14.631)(-37.819,-18.452)(-48.568,-20.785)(-60.500,-21.321)(-73.430,-22.590)(-85.165,-23.199)(-96.380,-26.799)(-105.412,-31.886)(-113.065,-34.908)(-123.630,-37.686)(-135.358,-42.234)(-148.845,-47.493)};
\drawtraj{(0.034,-0.253)(-23.668,12.591)(-48.935,24.188)(-73.755,35.178)(-96.351,48.024)(-119.475,61.893)(-142.899,77.819)(-169.664,94.670)(-198.634,112.376)(-228.067,128.756)(-257.784,146.332)(-288.337,164.907)(-315.182,184.849)(-338.898,206.604)(-362.154,228.010)};
\drawtraj{(0.084,-0.172)(8.298,7.999)(17.356,16.378)(28.594,24.775)(39.200,34.846)(49.449,45.623)(60.424,56.703)(70.325,68.696)(78.586,80.940)(87.233,93.156)(97.118,108.403)(106.815,124.780)(115.820,144.076)(126.707,168.234)(137.722,197.182)};


==> fig/data/data__evaluation_gevo_dtt_results_anees.tex <==
\drawkf\plotcommand{(3,1.093)(6,1.317)(9,1.278)(12,1.362)(15,1.334)};
\drawci\plotcommand{(3,0.524)(6,0.626)(9,0.586)(12,0.621)(15,0.609)};
\drawle\plotcommand{(3,0.991)(6,1.013)(9,0.972)(12,1.003)(15,1.017)};
\drawdca\plotcommand{(3,0.683)(6,0.669)(9,0.705)(12,0.756)(15,0.743)};

==> fig/data/data__evaluation_gevo_dtt_results_coin.tex <==
\drawkf\plotcommand{(3,1.334)(6,1.843)(9,1.585)(12,1.764)(15,1.869)};
\drawci\plotcommand{(3,0.605)(6,0.840)(9,0.768)(12,0.822)(15,0.756)};
\drawle\plotcommand{(3,1.146)(6,1.224)(9,1.103)(12,1.136)(15,1.187)};
\drawdca\plotcommand{(3,0.787)(6,0.817)(9,0.790)(12,0.848)(15,0.867)};

==> fig/data/data__evaluation_gevo_dtt_results_rmtr.tex <==
\drawkf\plotcommand{(3,1.128)(6,1.128)(9,1.125)(12,1.125)(15,1.125)};
\drawci\plotcommand{(3,1.063)(6,1.087)(9,1.093)(12,1.092)(15,1.092)};
\drawle\plotcommand{(3,1.001)(6,1.000)(9,1.000)(12,1.000)(15,1.000)};
\drawdca\plotcommand{(3,1.407)(6,1.400)(9,1.355)(12,1.348)(15,1.347)};


==> fig/data/data__evaluation_gevo_fusion_example_results_anees.tex <==
\drawdkf[solid]\plotcommand{(0.025,1)(0.075,1.000)(0.125,1)(0.175,1.000)(0.225,1)(0.275,1)(0.325,1.000)(0.375,1)(0.425,1)(0.475,1.000)(0.525,1)(0.575,1)(0.625,1)(0.675,1.000)(0.725,1.000)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1.000)};
\drawci[solid]\plotcommand{(0.025,0.777)(0.075,0.795)(0.125,0.815)(0.175,0.836)(0.225,0.858)(0.275,0.868)(0.325,0.875)(0.375,0.887)(0.425,0.902)(0.475,0.920)(0.525,0.944)(0.575,0.973)(0.625,1.000)(0.675,1.000)(0.725,1.000)(0.775,1.000)(0.825,1.000)(0.875,1.000)(0.925,1.000)(0.975,1.000)};
\drawle[solid]\plotcommand{(0.025,1)(0.075,1)(0.125,1.000)(0.175,1.000)(0.225,1.000)(0.275,1)(0.325,1)(0.375,1)(0.425,1.000)(0.475,1)(0.525,1.000)(0.575,1)(0.625,1.000)(0.675,1.000)(0.725,1)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1)};
\drawnkf[solid]\plotcommand{(0.025,1.003)(0.075,1.009)(0.125,1.015)(0.175,1.020)(0.225,1.020)(0.275,1.025)(0.325,1.031)(0.375,1.036)(0.425,1.042)(0.475,1.049)(0.525,1.056)(0.575,1.063)(0.625,1.071)(0.675,1.080)(0.725,1.090)(0.775,1.100)(0.825,1.112)(0.875,1.125)(0.925,1.140)(0.975,1.157)};
\drawdkf[dashed]\plotcommand{(0.025,1)(0.075,1)(0.125,1)(0.175,1)(0.225,1)(0.275,1)(0.325,1)(0.375,1.000)(0.425,1)(0.475,1)(0.525,1)(0.575,1)(0.625,1)(0.675,1.000)(0.725,1.000)(0.775,1.000)(0.825,1)(0.875,1.000)(0.925,1)(0.975,1)};
\drawci[dashed]\plotcommand{(0.025,0.611)(0.075,0.618)(0.125,0.627)(0.175,0.637)(0.225,0.648)(0.275,0.660)(0.325,0.675)(0.375,0.691)(0.425,0.709)(0.475,0.730)(0.525,0.755)(0.575,0.784)(0.625,0.819)(0.675,0.862)(0.725,0.916)(0.775,0.989)(0.825,1.000)(0.875,1.000)(0.925,1.000)(0.975,1.000)};
\drawle[dashed]\plotcommand{(0.025,1.000)(0.075,1)(0.125,1.000)(0.175,1.000)(0.225,1.000)(0.275,1)(0.325,1.000)(0.375,1)(0.425,1)(0.475,1)(0.525,1.000)(0.575,1)(0.625,1)(0.675,1.000)(0.725,1)(0.775,1)(0.825,1)(0.875,1.000)(0.925,1)(0.975,1.000)};
\drawnkf[dashed]\plotcommand{(0.025,1.005)(0.075,1.015)(0.125,1.026)(0.175,1.037)(0.225,1.048)(0.275,1.059)(0.325,1.071)(0.375,1.084)(0.425,1.097)(0.475,1.111)(0.525,1.126)(0.575,1.142)(0.625,1.158)(0.675,1.176)(0.725,1.195)(0.775,1.215)(0.825,1.237)(0.875,1.260)(0.925,1.286)(0.975,1.316)};
\drawdkf[dotted]\plotcommand{(0.025,1)(0.075,1.000)(0.125,1)(0.175,1.000)(0.225,1)(0.275,1)(0.325,1)(0.375,1)(0.425,1)(0.475,1.000)(0.525,1)(0.575,1)(0.625,1)(0.675,1)(0.725,1)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1)};
\drawci[dotted]\plotcommand{(0.025,0.534)(0.075,0.557)(0.125,0.579)(0.175,0.598)(0.225,0.617)(0.275,0.635)(0.325,0.654)(0.375,0.672)(0.425,0.690)(0.475,0.706)(0.525,0.724)(0.575,0.748)(0.625,0.775)(0.675,0.809)(0.725,0.850)(0.775,0.905)(0.825,0.981)(0.875,1.000)(0.925,1.000)(0.975,1.000)};
\drawle[dotted]\plotcommand{(0.025,1.000)(0.075,1)(0.125,1.000)(0.175,1)(0.225,1.000)(0.275,1)(0.325,1.000)(0.375,1.000)(0.425,1)(0.475,1)(0.525,1.000)(0.575,1)(0.625,1.000)(0.675,1.000)(0.725,1)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1.000)};
\drawnkf[dotted]\plotcommand{(0.025,1.019)(0.075,1.052)(0.125,1.080)(0.175,1.106)(0.225,1.129)(0.275,1.151)(0.325,1.171)(0.375,1.188)(0.425,1.196)(0.475,1.208)(0.525,1.225)(0.575,1.244)(0.625,1.264)(0.675,1.286)(0.725,1.311)(0.775,1.339)(0.825,1.369)(0.875,1.402)(0.925,1.437)(0.975,1.476)};


==> fig/data/data__evaluation_gevo_fusion_example_results_coin.tex <==
\drawdkf[solid]\plotcommand{(0.025,1)(0.075,1)(0.125,1)(0.175,1)(0.225,1)(0.275,1)(0.325,1)(0.375,1)(0.425,1)(0.475,1)(0.525,1)(0.575,1)(0.625,1)(0.675,1)(0.725,1)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1)};
\drawci[solid]\plotcommand{(0.025,0.869)(0.075,0.876)(0.125,0.884)(0.175,0.895)(0.225,0.906)(0.275,0.906)(0.325,0.907)(0.375,0.914)(0.425,0.923)(0.475,0.937)(0.525,0.954)(0.575,0.977)(0.625,1.000)(0.675,1.000)(0.725,1.000)(0.775,1.000)(0.825,1.000)(0.875,1.000)(0.925,1.000)(0.975,1.000)};
\drawle[solid]\plotcommand{(0.025,1.004)(0.075,1.011)(0.125,1.017)(0.175,1.028)(0.225,1.036)(0.275,1.038)(0.325,1.042)(0.375,1.045)(0.425,1.047)(0.475,1.048)(0.525,1.050)(0.575,1.050)(0.625,1.050)(0.675,1.049)(0.725,1.047)(0.775,1.044)(0.825,1.038)(0.875,1.031)(0.925,1.021)(0.975,1.007)};
\drawnkf[solid]\plotcommand{(0.025,1.018)(0.075,1.054)(0.125,1.090)(0.175,1.124)(0.225,1.125)(0.275,1.155)(0.325,1.187)(0.375,1.220)(0.425,1.256)(0.475,1.295)(0.525,1.336)(0.575,1.381)(0.625,1.429)(0.675,1.481)(0.725,1.539)(0.775,1.602)(0.825,1.673)(0.875,1.752)(0.925,1.841)(0.975,1.943)};
\drawdkf[dashed]\plotcommand{(0.025,1)(0.075,1)(0.125,1)(0.175,1)(0.225,1)(0.275,1)(0.325,1)(0.375,1)(0.425,1)(0.475,1)(0.525,1)(0.575,1)(0.625,1)(0.675,1)(0.725,1)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1)};
\drawci[dashed]\plotcommand{(0.025,0.735)(0.075,0.729)(0.125,0.726)(0.175,0.725)(0.225,0.726)(0.275,0.730)(0.325,0.735)(0.375,0.742)(0.425,0.752)(0.475,0.765)(0.525,0.782)(0.575,0.804)(0.625,0.832)(0.675,0.870)(0.725,0.925)(0.775,0.991)(0.825,1.000)(0.875,1.000)(0.925,1.000)(0.975,1.000)};
\drawle[dashed]\plotcommand{(0.025,1.006)(0.075,1.017)(0.125,1.026)(0.175,1.033)(0.225,1.039)(0.275,1.044)(0.325,1.047)(0.375,1.050)(0.425,1.052)(0.475,1.054)(0.525,1.054)(0.575,1.054)(0.625,1.054)(0.675,1.052)(0.725,1.049)(0.775,1.045)(0.825,1.040)(0.875,1.032)(0.925,1.021)(0.975,1.006)};
\drawnkf[dashed]\plotcommand{(0.025,1.018)(0.075,1.054)(0.125,1.090)(0.175,1.127)(0.225,1.165)(0.275,1.204)(0.325,1.245)(0.375,1.287)(0.425,1.331)(0.475,1.377)(0.525,1.425)(0.575,1.474)(0.625,1.525)(0.675,1.579)(0.725,1.634)(0.775,1.692)(0.825,1.752)(0.875,1.814)(0.925,1.878)(0.975,1.952)};
\drawdkf[dotted]\plotcommand{(0.025,1)(0.075,1)(0.125,1)(0.175,1)(0.225,1)(0.275,1)(0.325,1)(0.375,1)(0.425,1)(0.475,1)(0.525,1)(0.575,1)(0.625,1)(0.675,1)(0.725,1)(0.775,1)(0.825,1)(0.875,1)(0.925,1)(0.975,1.000)};
\drawci[dotted]\plotcommand{(0.025,0.613)(0.075,0.625)(0.125,0.663)(0.175,0.712)(0.225,0.753)(0.275,0.788)(0.325,0.816)(0.375,0.840)(0.425,0.854)(0.475,0.848)(0.525,0.852)(0.575,0.867)(0.625,0.883)(0.675,0.902)(0.725,0.925)(0.775,0.954)(0.825,0.991)(0.875,1.000)(0.925,1.000)(0.975,1.000)};
\drawle[dotted]\plotcommand{(0.025,1.009)(0.075,1.023)(0.125,1.034)(0.175,1.043)(0.225,1.049)(0.275,1.055)(0.325,1.059)(0.375,1.061)(0.425,1.063)(0.475,1.064)(0.525,1.064)(0.575,1.064)(0.625,1.062)(0.675,1.059)(0.725,1.055)(0.775,1.050)(0.825,1.044)(0.875,1.035)(0.925,1.023)(0.975,1.008)};
\drawnkf[dotted]\plotcommand{(0.025,1.081)(0.075,1.218)(0.125,1.327)(0.175,1.417)(0.225,1.491)(0.275,1.552)(0.325,1.601)(0.375,1.629)(0.425,1.596)(0.475,1.580)(0.525,1.598)(0.575,1.619)(0.625,1.642)(0.675,1.672)(0.725,1.709)(0.775,1.753)(0.825,1.802)(0.875,1.855)(0.925,1.911)(0.975,1.970)};


==> fig/data/data__evaluation_gevo_fusion_example_results_rmtr.tex <==
\drawdkf[solid]\plotcommand{(0.025,1.000)(0.075,1.000)(0.125,1.000)(0.175,0.999)(0.225,0.998)(0.275,0.998)(0.325,0.997)(0.375,0.997)(0.425,0.996)(0.475,0.996)(0.525,0.995)(0.575,0.995)(0.625,0.995)(0.675,0.994)(0.725,0.994)(0.775,0.994)(0.825,0.994)(0.875,0.995)(0.925,0.996)(0.975,0.998)};
\drawci[solid]\plotcommand{(0.025,1.155)(0.075,1.155)(0.125,1.153)(0.175,1.151)(0.225,1.163)(0.275,1.175)(0.325,1.177)(0.375,1.177)(0.425,1.175)(0.475,1.171)(0.525,1.165)(0.575,1.157)(0.625,1.145)(0.675,1.132)(0.725,1.117)(0.775,1.100)(0.825,1.082)(0.875,1.062)(0.925,1.039)(0.975,1.014)};
\drawle[solid]\plotcommand{(0.025,1.001)(0.075,1.000)(0.125,1.000)(0.175,1.001)(0.225,1.003)(0.275,1.003)(0.325,1.004)(0.375,1.004)(0.425,1.004)(0.475,1.004)(0.525,1.004)(0.575,1.004)(0.625,1.004)(0.675,1.004)(0.725,1.003)(0.775,1.003)(0.825,1.003)(0.875,1.003)(0.925,1.002)(0.975,1.001)};
\drawnkf[solid]\plotcommand{(0.025,1.000)(0.075,0.999)(0.125,0.999)(0.175,0.998)(0.225,0.996)(0.275,0.994)(0.325,0.992)(0.375,0.990)(0.425,0.988)(0.475,0.985)(0.525,0.982)(0.575,0.979)(0.625,0.975)(0.675,0.970)(0.725,0.965)(0.775,0.959)(0.825,0.952)(0.875,0.943)(0.925,0.932)(0.975,0.919)};
\drawdkf[dashed]\plotcommand{(0.025,0.999)(0.075,0.998)(0.125,0.998)(0.175,0.997)(0.225,0.996)(0.275,0.995)(0.325,0.995)(0.375,0.994)(0.425,0.993)(0.475,0.993)(0.525,0.992)(0.575,0.992)(0.625,0.992)(0.675,0.992)(0.725,0.992)(0.775,0.992)(0.825,0.993)(0.875,0.994)(0.925,0.995)(0.975,0.998)};
\drawci[dashed]\plotcommand{(0.025,1.297)(0.075,1.302)(0.125,1.305)(0.175,1.305)(0.225,1.304)(0.275,1.301)(0.325,1.296)(0.375,1.290)(0.425,1.282)(0.475,1.273)(0.525,1.261)(0.575,1.248)(0.625,1.232)(0.675,1.212)(0.725,1.189)(0.775,1.160)(0.825,1.127)(0.875,1.092)(0.925,1.057)(0.975,1.019)};
\drawle[dashed]\plotcommand{(0.025,1.007)(0.075,1.006)(0.125,1.006)(0.175,1.006)(0.225,1.006)(0.275,1.006)(0.325,1.006)(0.375,1.006)(0.425,1.006)(0.475,1.006)(0.525,1.005)(0.575,1.005)(0.625,1.005)(0.675,1.005)(0.725,1.005)(0.775,1.004)(0.825,1.004)(0.875,1.003)(0.925,1.002)(0.975,1.001)};
\drawnkf[dashed]\plotcommand{(0.025,0.999)(0.075,0.996)(0.125,0.994)(0.175,0.991)(0.225,0.988)(0.275,0.984)(0.325,0.981)(0.375,0.976)(0.425,0.972)(0.475,0.967)(0.525,0.962)(0.575,0.956)(0.625,0.950)(0.675,0.943)(0.725,0.935)(0.775,0.926)(0.825,0.916)(0.875,0.904)(0.925,0.888)(0.975,0.863)};
\drawdkf[dotted]\plotcommand{(0.025,0.996)(0.075,0.991)(0.125,0.989)(0.175,0.988)(0.225,0.988)(0.275,0.987)(0.325,0.987)(0.375,0.987)(0.425,0.986)(0.475,0.985)(0.525,0.984)(0.575,0.983)(0.625,0.983)(0.675,0.983)(0.725,0.984)(0.775,0.985)(0.825,0.987)(0.875,0.989)(0.925,0.992)(0.975,0.997)};
\drawci[dotted]\plotcommand{(0.025,1.378)(0.075,1.357)(0.125,1.342)(0.175,1.330)(0.225,1.319)(0.275,1.310)(0.325,1.301)(0.375,1.292)(0.425,1.282)(0.475,1.271)(0.525,1.258)(0.575,1.244)(0.625,1.228)(0.675,1.209)(0.725,1.188)(0.775,1.163)(0.825,1.132)(0.875,1.096)(0.925,1.059)(0.975,1.020)};
\drawle[dotted]\plotcommand{(0.025,1.038)(0.075,1.029)(0.125,1.024)(0.175,1.020)(0.225,1.017)(0.275,1.015)(0.325,1.014)(0.375,1.013)(0.425,1.012)(0.475,1.011)(0.525,1.011)(0.575,1.010)(0.625,1.010)(0.675,1.009)(0.725,1.008)(0.775,1.008)(0.825,1.006)(0.875,1.005)(0.925,1.003)(0.975,1.001)};
\drawnkf[dotted]\plotcommand{(0.025,0.991)(0.075,0.979)(0.125,0.971)(0.175,0.964)(0.225,0.959)(0.275,0.954)(0.325,0.950)(0.375,0.945)(0.425,0.940)(0.475,0.933)(0.525,0.925)(0.575,0.917)(0.625,0.908)(0.675,0.899)(0.725,0.888)(0.775,0.877)(0.825,0.865)(0.875,0.851)(0.925,0.835)(0.975,0.813)};


==> fig/data/data__evaluation_pco_dtt_results_anees.tex <==
\drawkfpco\plotcommand{(3,1.236)(6,1.300)(9,1.269)(12,1.331)(15,1.332)};
\drawcipco\plotcommand{(3,0.873)(6,0.793)(9,0.807)(12,0.856)(15,0.850)};
\drawicipco\plotcommand{(3,0.917)(6,0.970)(9,0.946)(12,0.974)(15,0.984)};
\drawlepco\plotcommand{(3,0.976)(6,0.972)(9,0.956)(12,0.991)(15,0.989)};


==> fig/data/data__evaluation_pco_dtt_results_coin.tex <==
\drawkfpco\plotcommand{(3,1.796)(6,2.035)(9,1.900)(12,2.022)(15,1.999)};
\drawcipco\plotcommand{(3,0.972)(6,0.953)(9,0.913)(12,1.004)(15,1.000)};
\drawicipco\plotcommand{(3,1.195)(6,1.593)(9,1.483)(12,1.468)(15,1.430)};
\drawlepco\plotcommand{(3,1.314)(6,1.606)(9,1.511)(12,1.464)(15,1.427)};


==> fig/data/data__evaluation_pco_dtt_results_rmtr.tex <==
\drawkfpco\plotcommand{(3,1.984)(6,1.708)(9,1.696)(12,1.697)(15,1.697)};
\drawcipco\plotcommand{(3,1.427)(6,1.390)(9,1.342)(12,1.339)(15,1.338)};
\drawlepco\plotcommand{(3,1.712)(6,1.352)(9,1.339)(12,1.340)(15,1.340)};


==> fig/data/data__gevoci_cra_nx=6_e=0.00010.tex <==
\drawfreq{clrm1} plot coordinates {(1,-2.987163)(2,-0.678598)(3,-0.429168)(4,-0.702546)(5,-1.022917)(6,-1.311269)(7,-1.570959)(8,-1.802582)(9,-2.004453)(10,-2.194907)(11,-2.364516)(12,-2.513003)(13,-2.657775)(14,-2.806319)(15,-2.949620)(16,-3.067019)(17,-3.216811)(18,-3.287350)(19,-3.396856)(20,-3.484126)(21,-3.616185)(22,-3.737549)(23,-3.821023)(24,-3.982967)(25,-3.974694)(26,-4.086186)(27,-4.180456)(28,-4.346787)(29,-4.522879)(30,-4.408935)(31,-4.657577)(32,-4.638272)(33,-4.744727)(34,-4.886057)(35,-4.886057)(36,-5.096910)(37,-5.221849)(38,-5.154902)(39,-5.154902)(40,-6.000000)(41,-5.154902)(42,-5.301030)(43,-5.698970)(44,-10.000000)(45,-5.698970)(46,-5.698970)(47,-5.698970)(48,-10.000000)(49,-6.000000)};
\drawfreq{clrm2} plot coordinates {(1,-3.336299)(2,-0.543971)(3,-0.313819)(4,-0.774975)(5,-1.375697)(6,-1.937869)(7,-2.427709)(8,-2.836540)(9,-3.151811)(10,-3.446117)(11,-3.692504)(12,-3.962574)(13,-4.214670)(14,-4.408935)(15,-4.619789)(16,-4.769551)(17,-4.853872)(18,-5.154902)(19,-5.397940)(20,-6.000000)(21,-5.698970)(22,-6.000000)(23,-6.000000)(24,-10.000000)(25,-10.000000)(26,-10.000000)(27,-10.000000)(28,-10.000000)(29,-6.000000)(30,-10.000000)(31,-10.000000)(32,-10.000000)(33,-10.000000)(34,-6.000000)};
\drawfreq{clrm3} plot coordinates {(1,-1.161101)(2,-0.208674)(3,-0.571174)(4,-1.423716)(5,-2.298259)(6,-3.013228)(7,-3.649752)(8,-4.036212)(9,-4.443697)(10,-4.886057)(11,-4.920819)(12,-5.522879)(13,-5.301030)(14,-6.000000)(15,-6.000000)(16,-10.000000)(17,-10.000000)(18,-10.000000)(19,-10.000000)(20,-10.000000)(21,-10.000000)(22,-6.000000)};
\drawfreq{clrm4} plot coordinates {(1,-0.450176)(2,-0.217889)(3,-1.427919)(4,-2.648590)(5,-3.677781)(6,-4.387216)(7,-5.301030)(8,-6.000000)};


==> fig/data/data__gevoci_cra_nx=6_e=0.00100.tex <==
\drawfreq{clrm1} plot coordinates {(1,-2.462181)(2,-0.365487)(3,-0.475041)(4,-0.889087)(5,-1.276520)(6,-1.623587)(7,-1.924964)(8,-2.217599)(9,-2.486516)(10,-2.799423)(11,-3.064493)(12,-3.332547)(13,-3.551294)(14,-3.764472)(15,-4.000000)(16,-4.251812)(17,-4.619789)(18,-4.638272)(19,-5.154902)(20,-5.522879)(21,-5.522879)(22,-10)(23,-10)(24,-10)(25,-10)(26,-10)(27,-10)(28,-10)(29,-10)(30,-10)(31,-10)(32,-10)(33,-10)(34,-10)(35,-10)(36,-10)(37,-10)(38,-10)(39,-10)(40,-10)(41,-10)(42,-10)(43,-10)(44,-10)(45,-10)(46,-10)(47,-10)(48,-10)(49,-10)(50,-6.000000)};
\drawfreq{clrm2} plot coordinates {(1,-2.110362)(2,-0.203539)(3,-0.501412)(4,-1.368708)(5,-2.201902)(6,-2.821023)(7,-3.366532)(8,-3.882729)(9,-4.356547)(10,-4.769551)(11,-5.522879)(12,-5.522879)(13,-6.000000)(14,-10)(15,-6.000000)};
\drawfreq{clrm3} plot coordinates {(1,-0.617860)(2,-0.163466)(3,-1.163138)(4,-2.456553)(5,-3.464706)(6,-4.193820)(7,-5.096910)(8,-5.301030)};
\drawfreq{clrm4} plot coordinates {(1,-0.128877)(2,-0.597434)(3,-2.402305)(4,-3.910095)(5,-5.045757)(6,-6.000000)};


==> fig/data/data__gevoci_cra_nx=9_e=0.00010.tex <==
\drawfreq{clrm1} plot coordinates {(1,-4.602060)(2,-0.962677)(3,-0.426646)(4,-0.612052)(5,-0.918671)(6,-1.212497)(7,-1.471353)(8,-1.714555)(9,-1.917646)(10,-2.119015)(11,-2.289544)(12,-2.460673)(13,-2.625252)(14,-2.769807)(15,-2.891773)(16,-3.045757)(17,-3.164309)(18,-3.307153)(19,-3.443697)(20,-3.567031)(21,-3.640165)(22,-3.785156)(23,-3.906578)(24,-4.055517)(25,-4.102373)(26,-4.259637)(27,-4.346787)(28,-4.494850)(29,-4.481486)(30,-4.677781)(31,-4.721246)(32,-4.853872)(33,-4.823909)(34,-5.522879)(35,-5.045757)(36,-5.522879)(37,-5.698970)(38,-5.522879)(39,-5.397940)(40,-5.522879)(41,-10)(42,-5.698970)(43,-10)(44,-10)(45,-10)(46,-10)(47,-10)(48,-10)(49,-10)(50,-6.000000)};
\drawfreq{clrm2} plot coordinates {(2,-1.203086)(3,-0.274496)(4,-0.514675)(5,-1.136517)(6,-1.751144)(7,-2.278932)(8,-2.679231)(9,-3.049149)(10,-3.333482)(11,-3.632644)(12,-3.777284)(13,-4.036212)(14,-4.267606)(15,-4.397940)(16,-4.619789)(17,-4.744727)(18,-5.000000)(19,-5.301030)(20,-5.221849)(21,-5.698970)(22,-5.698970)(23,-10)(24,-6.000000)(25,-10)(26,-6.000000)};
\drawfreq{clrm3} plot coordinates {(2,-0.837427)(3,-0.170196)(4,-0.794390)(5,-1.811072)(6,-2.696588)(7,-3.302771)(8,-3.785156)(9,-4.173925)(10,-4.494850)(11,-4.638272)(12,-4.920819)(13,-5.221849)(14,-5.397940)(15,-6.000000)(16,-10)(17,-6.000000)};
\drawfreq{clrm4} plot coordinates {(1,-2.860436)(2,-0.344935)(3,-0.290538)(4,-1.482237)(5,-2.871924)(6,-3.892790)(7,-4.468521)(8,-4.886057)(9,-5.698970)(10,-5.301030)(11,-6.000000)(12,-6.000000)(13,-6.000000)};


==> fig/data/data__gevoci_cra_nx=9_e=0.00100.tex <==
\drawfreq{clrm1} plot coordinates {(1,-3.987163)(2,-0.488032)(3,-0.398303)(4,-0.794704)(5,-1.191654)(6,-1.552656)(7,-1.905319)(8,-2.265520)(9,-2.631899)(10,-2.958607)(11,-3.236572)(12,-3.521434)(13,-3.847712)(14,-4.309804)(15,-4.769551)(16,-4.920819)(17,-5.301030)};
\drawfreq{clrm2} plot coordinates {(1,-6.000000)(2,-0.445908)(3,-0.255729)(4,-1.128094)(5,-2.017412)(6,-2.700275)(7,-3.257275)(8,-3.818156)(9,-4.187087)(10,-4.698970)(11,-5.221849)(12,-10)(13,-10)(14,-10)(15,-10)(16,-10)(17,-10)(18,-10)(19,-10)(20,-10)(21,-10)(22,-10)(23,-10)(24,-10)(25,-10)(26,-10)(27,-10)(28,-10)(29,-10)(30,-10)(31,-10)(32,-10)(33,-10)(34,-10)(35,-10)(36,-10)(37,-10)(38,-10)(39,-10)(40,-10)(41,-10)(42,-10)(43,-10)(44,-10)(45,-10)(46,-10)(47,-10)(48,-10)(49,-10)(50,-6.000000)};
\drawfreq{clrm3} plot coordinates {(1,-4.130768)(2,-0.195944)(3,-0.454735)(4,-1.946115)(5,-3.182435)(6,-4.055517)(7,-4.823909)(8,-5.698970)};
\drawfreq{clrm4} plot coordinates {(1,-1.716292)(2,-0.045778)(3,-1.095831)(4,-3.217527)(5,-4.744727)(6,-5.698970)};

